LLM Chemistry Estimation for Multi-LLM Recommendation

Multi-LLM collaboration promises accurate, robust, and context-aware solutions, yet existing approaches rely on implicit selection and output assessment without analyzing whether collaborating models truly complement or conflict. We introduce LLM Chemistry -- a framework that measures when LLM combinations exhibit synergistic or antagonistic behaviors that shape collective performance beyond individual capabilities. We formalize the notion of chemistry among LLMs, propose algorithms that quantify it by analyzing interaction dependencies, and recommend optimal model ensembles accordingly. Our theoretical analysis shows that chemistry among collaborating LLMs is most evident under heterogeneous model profiles, with its outcome impact shaped by task type, group size, and complexity. Evaluation on classification, summarization, and program repair tasks provides initial evidence for these task-dependent effects, thereby reinforcing our theoretical results. This establishes LLM Chemistry as both a diagnostic factor in multi-LLM systems and a foundation for ensemble recommendation.

==> content/sections/02-preliminaries.tex <==
%
\section{Preliminaries}%
\label{subsec:prelimns}

\textbf{Basic Concepts}. Let $Q$ be a query that needs answering. Suppose we
have a group of candidate LLMs (denoted by $S$), each with recorded past
performance (e.g., accuracy of LLMs and a quality score for their outputs). Our
objective is threefold: (1) to understand how these LLMs interact---i.e., to
estimate their \textit{chemistry}---when jointly answering $Q$, (2) to assess
the performance impact of their interactions, and (3) to determine the optimal
collaborative configuration for effectively answering $Q$.
%
%
%
%
%

For any given LLM configuration $X \subseteq S$ that was chosen to answer $Q$,
we use $O$ to denote the outputs generated by the LLMs in $X$. We also introduce
$\mathit{cost}(X)$ and $\mathit{used}(X)$ to denote the cost and the LLMs in $X$
that actually generated an output for $Q$. Hence, $\mathit{used}(X) \subseteq X$
by definition, and $X\;-\;\mathit{used}(X)$ may be non-empty if some LLMs are
not used to answer $Q$.

A $\mathit{cost}(S)$ is defined as follows: Given $O = \{o_1, o_2, \ldots,
o_n\}$ for $n > 0$, where each $o_i$ has a quality score $q_i$ with range $[0.0,
10.0]$, each LLM in $S$ producing $o_i$ has accuracy $a_i$ with range $[0.0,
1.0]$, and a weight $w_i\;=\;1/i$~\footnote{The weights are positive real
numbers that are inversely proportional to the rank of the answers. Intuitively,
top-ranked answers dominate the total cost.}. Since quality $q_i$ is between
$0.0$ and $10.0$, we normalize it to a $[0,1]$ range to match accuracy $a_i$:
$q_i^{\mathit{norm}} = \frac{q_i}{10}$, where $q_i^{\mathit{norm}} \in [0,1]$.
Accordingly, a high normalized quality $(q_i^{\mathit{norm}}\approx 1)$ and high
accuracy ($a_i\approx 1$) produce low penalties. Conversely, low values in
either measurement produce higher penalties. Thus, the penalty per answer
naturally becomes: $\mathit{penalty}_i = (1 - q_i^{\mathit{norm}}) \cdot (1 -
a_i)$. The total cost over all $n$ answers in $O$, weighted by $w_i$, is:

%
%

\begin{equation} %
	\label{eq:cost}
	C_{total} = \sum_{i=1}^{n} w_i \cdot \left(1 - q_i^{\mathit{norm}}\right) \cdot
  (1 - a_i)
\end{equation}

The best-case scenario ($q_i = 10, a_i = 1$): penalty is $0$. Lower values in
either quality or accuracy, increase the penalty (thus, the total cost). E.g.,
let's say we have three likely answers:\medskip

%
%
%
%
%
\begin{table}[h]
\centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{c|c|c|c}
\hline
\textbf{Rank ($i$)} & \textbf{Quality ($q_i$, out of 10)} & \textbf{Accuracy ($a_i$) [0,1]} & \textbf{Weight ($w_i = 1/i$)} \\
\hline
1 & 9.0 & 0.90 & 1.00 \\
2 & 8.0 & 0.80 & 0.50 \\
3 & 7.0 & 0.70 & 0.33 \\
\hline
\end{tabular}
}
\caption{Example ranking table with quality, accuracy, and inverse rank weight.}
\label{tab:ranking}
\end{table}

Then the total cost is:
%
%
%
%
\begin{align*}
C_{\mathit{total}} &= (1.00 \cdot (1 - 0.9) \cdot (1 - 0.9)) \nonumber \\
&\quad + (0.50 \cdot (1 - 0.8) \cdot (1 - 0.8)) \nonumber \\
&\quad + (0.33 \cdot (1 - 0.7) \cdot (1 - 0.7))
\end{align*}

Thus:
\[
C_{\mathit{total}} \approx 0.01 + 0.02 + 0.0297 = 0.0597
\]\smallskip
\vspace{-0.4em}

This total cost number shows that a low penalty is applied for a
good-quality/high-accuracy answer at the top, and higher penalties are applied
as quality and accuracy decrease down the rank. This insight into the cost
function forms the basis for defining the \textit{benefit} of LLMs in a set.

In this paper, we compute quality scores $q_i$ and accuracy $a_i$ using a
consensus-based approach inspired by the \textit{Vancouver crowdsourcing
algorithm}~\citep{de2014crowdgrader}. We apply a \textit{Minimum Variance Linear
Estimator} (MVLE) to iteratively infer both the consensus score for each
response and the variance associated with each LLM. The consensus score reflects
the estimated quality of the response $q_i$, assigning higher values to models
whose outputs consistently align with low-variance consensus across items. In
this setup, the \textit{inverse variance} serves as a proxy for review accuracy.

We compute a continuous $a_i$ for an LLM by combining its generation accuracy
and review accuracy values. The union of these two complementary signals
provides a unified indicator of task performance for each individual LLM. In
this paper, this indicator primarily emphasizes ($75$\%) each LLM's demonstrated
accuracy in generating correct responses, complemented by a moderate emphasis
($25$\%) on independently assessed reviewing accuracy. If no ground truth is
available---the emphasis is flipped---i.e., $75$\% weight on review accuracy,
$25$\% on generation accuracy. For example, on a fake news classification task
with o3-mini, generation accuracy is $1.0$ and review accuracy $0.846$, giving
$a_i = 0.962$.

%
%
%
%

We chose MVLE over traditional voting methods to compute $q_i$ and $a_i$ for its
statistical grounding, robustness to noise and unreliable responses, and ability
to iteratively refine both consensus scores and model reliability estimates.

%
%

\textbf{Benefit of LLMs in a Set}. Given \eref{eq:cost} and two disjoint sets
$X$, $Y \subseteq S$, we define the \emph{benefit} of an individual LLM in a set
of LLMs as the difference in performance cost if LLMs in $Y$ are selected in
addition to the LLMs in $X$. Formally,

\begin{definition}[Benefit]
Given two LLM sets $X$, $Y \subseteq S$ and a query $Q$, the benefit of $X$
with respect to $Y$ and $Q$ is defined as $\mathit{benefit}(X,\,Y) =
\mathit{cost}(Y) - \mathit{cost}(X\;\cup\;Y)$.
\end{definition}

The value of $\mathit{benefit}(X, Y)$ can be negative if adding $X$ to $Y$
increases the total cost, indicating that adding $X$ degrades rather than
improves performance. \suggest{While the notion of benefit captures how
individual LLMs contribute to a set, it does not fully characterize the complex
interdependencies that emerge when multiple LLMs work together.} Understanding
when and how such degradations occur---and more generally, how LLMs influence
each other's effectiveness---is key to analyzing the chemistry between models.
In what follows, we define the \emph{LLM chemistry} to quantify such interaction
effects.

%
%

